A Well Balanced Reconstruction with Bounded Velocities and Low-Oscillation Slow Shocks for the Shallow Water Equations

Many numerical schemes for hyperbolic systems require a piecewise polynomial reconstruction of the cell averaged values, and to simulate perturbed steady states accurately we require a so called 'well balanced' reconstruction scheme. For the shallow water system this involves reconstructing in surface elevation, to which modifications must be made as the fluid depth becomes small to ensure positivity. We investigate the scheme proposed in Skevington (2021) though numerical experiments, demonstrating its ability to resolve steady and near steady states at high accuracy. We also present a modification to the scheme which enables the resolution of slowly moving shocks and dam break problems without compromising the well balanced property.

==> Templates/StandardMathsMacros.tex <==
%My macros for the math environment

\usepackage{xparse}
\makeatletter




%---BRACKETS----

%Normal brackets

\DeclarePairedDelimiter{\ppar}{\lparen}{\rparen}
\DeclarePairedDelimiter{\pang}{\langle}{\rangle}
\DeclarePairedDelimiter{\pbrc}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\pbrk}{\lbrack}{\rbrack}
\DeclarePairedDelimiter{\pgrp}{\lgroup}{\rgroup}

%Bracket-like structures

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\round}{\lfloor}{\rceil}

\DeclarePairedDelimiter{\eval@wdot}{.}{\rvert}
\NewDocumentCommand{\eval}{som}{%
	\IfBooleanTF{#1}
    	{\eval@wdot*{#3}}
   		{\IfNoValueTF{#2}{#3\rvert}{\eval@wdot[#2]{#3}}}%
}

\DeclarePairedDelimiterX{\setpred}[2]{\lbrace}{\rbrace}{\: #1 \: \delimsize\vert \: #2 \:}




%---OPERATORS---

\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\minmod}{minmod}
\DeclareMathOperator{\diag}{diag}




%---DIMENSIONLESS CONSTANTS---
%Define carefully, some of these are defined in the JFM template

%\Rey Reynolds number 
\ifdefined\Rey\else
	\newcommand\Rey{\mbox{\textit{Re}}}
\fi

%\Pran Prandtl number
\ifdefined\Pran\else
	\newcommand\Pran{\mbox{\textit{Pr}}} 
\fi

%\Pen Peclet number
\ifdefined\Pen\else
	\newcommand\Pen{\mbox{\textit{Pe}}}
\fi

%\Fro Froude number
\ifdefined\Fro\else
	\newcommand\Fro{\mbox{\textit{Fr}}}
\fi

%\Ric Richardson number
\ifdefined\Ric\else
	\newcommand\Ric{\mbox{\textit{Ri}}}
\fi




%---CALCULUS---
%Uses the calculus syntax from the Physics package with a few modifications
%
%For fractions p/q, following applies
%\frac{p}{q}, standard
%\frac*{p}{q}, flat
%\frac**{p}{q}, flat, autosize slash
%\frac*[\size]{p}{q}, flat, slash size of \size
%
%For differential d syntax is
%\dd*[power]{measure}
%Star removes spacing
%
%For derivative df/dx, stars the same as for \frac, optional argument the order of the derivative
%\dv(frac syntax here)[order]{f}{x}
%If wanting to use a flat derivative without sizing with order, then \dv*[][n]{f}{x}
%
%For partial derivative df/dx, use \pdv with syntax as for \dv
%NOT IMPLEMENTED YET Alternatively, for d^n f/dx_1 ... dx_n use
%\pdvm(frac syntax here){n}{f}{x_1}...{x_n}

%\frac
\let\frac@nostar\frac
\DeclarePairedDelimiterX{\frac@starwdot}[2]{.}{.}{#1 \delimsize/ #2}
\NewDocumentCommand{\frac@star}{somm}{%
	\IfBooleanTF{#1}
    	{\frac@starwdot*{#3}{#4}}
    	{\IfNoValueTF{#2}{#3/#4}{\frac@starwdot[#2]{#3}{#4}}}%
}
\renewcommand*\frac{\@ifstar{\frac@star}{\frac@nostar}}

%\dd
\NewDocumentCommand{\dd}{som}{%
	\IfBooleanF{#1}{\,}%
	\IfNoValueTF{#2}{%Check whether optional argument is given
		\textrm{d} #3%
	}{%
		\textrm{d}^{#2} #3%
	}%
	\IfBooleanF{#1}{\,}%
}

%\dv
\NewDocumentCommand\dv@nostar{O{}mm}{%
	\frac@nostar{\textrm{d}^{#1} #2}{{\textrm{d} #3}^{#1}}
}
\NewDocumentCommand{\dv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\textrm{d}^{#2} #4}{{\textrm{d} #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\textrm{d}^{#3} #4}{{\textrm{d} #5}^{#3}}%
		\else
			\frac*[#2]{\textrm{d}^{#3} #4}{{\textrm{d} #5}^{#3}}%
		\fi
	}%
}
\newcommand*\dv{\@ifstar{\dv@star}{\dv@nostar}}

%\pdv
\NewDocumentCommand\pdv@nostar{O{}mm}{%
	\frac@nostar{\partial^{#1} #2}{{\partial #3}^{#1}}
}
\NewDocumentCommand{\pdv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\partial^{#2} #4}{{\partial #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\else
			\frac*[#2]{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\fi
	}%
}
\newcommand*\pdv{\@ifstar{\pdv@star}{\pdv@nostar}}

%%\pdvm
%\NewDocumentCommand\pdvm@nostar@two{mmmm}{%
%	\frac{\partial^2 #2}{\partial #3 \partial #4}
%}
%\NewDocumentCommand{\pdvm@star@two}{sO{}mmm}{%
%	|#1,#2,#3,#4,#5|
%%	\IfBooleanTF{#2}{%
%%		\frac**{\partial^2 #4}{\partial #5 \partial #6}%
%%	}{%
%%		\if \relax\detokenize{#3}\relax
%%			\frac*{\partial^2 #4}{\partial #5 \partial #6}%
%%		\else
%%			\frac*[#3]{\partial^2 #4}{\partial #5 \partial #6}%
%%		\fi
%%	}%
%}
%\newcommand*\pdvm@nostar[1]{%
%	\ifnum #1=2
%		\pdvm@nostar@two%
%	\fi%
%}
%\newcommand*\pdvm@STAR[1]{%
%	\ifnum #1=2
%		\pdvm@nostar@two%
%	\fi%
%}
%\newcommand*\pdvm{\@ifstar{\pdvm@star}{\pdvm@nostar}}

%\def\pdvm@str@frac{frac}
%\def\pdvm@str@flat{flat}
%\def\pdvm@str@slsh{slsh}
%
%\NewDocumentCommand{\pdvm@two}{mmmmm}{
%	F|#1,#2,#3,#4,#5|
%}
%
%\newcommand*\pdvm@nostar[1]{%
%	A|#1| \:
%	\ifnum #1=2
%		\pdvm@two{\pdvm@str@frac}{}%
%	\fi%
%}
%\newcommand*\pdvm@star[2]{%
%	B%\abs{ #1 , #2 } \:
%%	\ifnum #2=2
%%		\pdvm@two{\pdvm@str@slsh}{#1}%
%%	\fi%
%}
%\newcommand*\pdvm@sstar[1]{%
%	C|#1| \:
%	\ifnum #1=2
%		\pdvm@two{\pdvm@str@flat}{}%
%	\fi%
%}
%
%\newcommand\pdvm@staropt[1][]{%
%	a| #1 | \:%
%	\if \relax\detokenize{#1}\relax
%		b%
%		\pdvm@star{}%
%	\else
%		c%
%		\pdvm@star{#1}%
%	\fi
%}
%\newcommand*\pdvm@STAR{\@ifstar{\pdvm@sstar}{\pdvm@staropt}}
%\newcommand*\pdvm{\@ifstar{\pdvm@STAR}{\pdvm@nostar}}


%---ORDER NOTATION---

%If order is used with an empty argument then dont use parenthesis
\newcommand{\order@text}[1]{	
	\if\relax\detokenize{#1}\relax% #1 is empty
	\else% #1 is nonempty
		\ppar*{#1}%\qty(#1)
	\fi
}

%Big O
\newcommand{\order}[1]{
	\mathcal{O}\order@text{#1}
}

%Little O
\newcommand{\lorder}[1]{
  	\mathchoice
    	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \displaystyle
    	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \textstyle
    	{{\scriptscriptstyle\mathcal{O}}\order@text{#1}}% \scriptstyle
    	{\scalebox{.6}{${\scriptscriptstyle\mathcal{O}}\order@text{#1}$}}%\scriptscriptstyle
  	}

%Big Theta
\newcommand{\Torder}[1]{
	\mathit{\Theta}\order@text{#1}
}




%---ASSORTED---

%Have equation span full width of collumn (good for equations in lists)
\newcommand{\eqnwide}{\displayindent0pt \displaywidth\textwidth}

%Use as 10^\nth
\newcommand{\nth}{\text{th}}

%Defined to be equal to
\newcommand{\eqdef}{\vcentcolon =}%{\stackrel{\mathrm{def}}{=}}

%Text style fraction
\newcommand{\textfrac}[2] {{\textstyle\frac{#1}{#2}}}

%Omitted dummy variable as a dot
\newcommand*\omitdummy{\mathchoice
	{\omitdummy@{\displaystyle}{0.6}}
	{\omitdummy@{\textstyle}{0.6}}
	{\omitdummy@{\scriptstyle}{0.7}}
	{\omitdummy@{\scriptscriptstyle}{0.8}}
}
\newcommand*\omitdummy@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}




%---ENVIRONMENTS---

%Like cases but with as many collumns as you like

\newenvironment{multicasesnobrac}[1][1]{%
%No braces
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\begin{array}{*{#1}{r@{}l}}
}{
	\end{array}
}
\newenvironment{multicases}[1][1]{%
%Left braced
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{r@{}l}}
}{
	\end{array}\right.
}
\newenvironment{multicasesd}[1][1]{%
%Left braced with display style
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{>{\displaystyle}{r}@{}>{\displaystyle}{l}}}
}{
	\end{array}\right.
}




%---SIDE BY SIDE SUBEQUATIONS---

%Multiple labeled equations on same line
\newlength{\sbsse@Wl}	%Width of left equation
\newlength{\sbsse@Wm}	%Width of mid text
\newlength{\sbsse@Wr}	%Width of right equation
\newlength{\sbsse@Wt}	%Width of tag
\newlength{\sbsse@We}	%Remaining width on line
\newlength{\sbsse@Wd}	%Remaining width divided into pieces

%Two equations side by side
\newcommand\sidebysidesubequations[6]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    midtext
	% #5    right subequation
	% #6    right label
  
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{\text{#4}}
	\def\sbsse@Er{#5}
	\def\sbsse@Et{(\ref*{#1}a,b)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space, and midtext if any
			\if\relax\detokenize{#4}\relax
				\setlength{\sbsse@Wd}{\sbsse@We/3}
				\hspace{\sbsse@Wd}
			\else
				\setlength{\sbsse@Wd}{\sbsse@We/4}
				\hspace{\sbsse@Wd}\sbsse@Em\hspace{\sbsse@Wd}
			\fi
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#6}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}

%Three equations side by side
\newcommand\sidebysidesubequationsT[7]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    mid subequation
	% #5	mid label
	% #6    right subequation
	% #7    right label
  
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{#4}
	\def\sbsse@Er{#6}
	\def\sbsse@Et{(\ref*{#1}a,b,c)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	\setlength{\sbsse@Wd}{\sbsse@We/4}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space
			\hspace{\sbsse@Wd}
			%Mid equation and label
			\sbsse@Em\refstepcounter{equation}\ltx@label{{#5}}
			%Space
			\hspace{\sbsse@Wd}
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#7}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}




\makeatother
